Exploring Interpretable LSTM Neural Networks over Multi-Variable Data

For recurrent neural networks trained on time series with target and exogenous variables, in addition to accurate prediction, it is also desired to provide interpretable insights into the data. In this paper, we explore the structure of LSTM recurrent neural networks to learn variable-wise hidden states, with the aim to capture different dynamics in multi-variable time series and distinguish the contribution of variables to the prediction. With these variable-wise hidden states, a mixture attention mechanism is proposed to model the generative process of the target. Then we develop associated training methods to jointly learn network parameters, variable and temporal importance w.r.t the prediction of the target variable. Extensive experiments on real datasets demonstrate enhanced prediction performance by capturing the dynamics of different variables. Meanwhile, we evaluate the interpretation results both qualitatively and quantitatively. It exhibits the prospect as an end-to-end framework for both forecasting and knowledge extraction over multi-variable data.

==> Exploring interpretable LSTM neural networks over multi-variable data/conclusion.tex <==
\section{Conclusion and Discussion}
In this paper, we explore the internal structures of LSTMs for interpretable prediction on multi-variable time series. 
Based on the hidden state matrix, we present two realizations i.e. IMV-Full and IMV-Tensor, which enable to infer and quantify variable importance and variable-wise temporal importance w.r.t. the target.
Extensive experiments provide insights into achieving superior prediction performance and importance interpretation for LSTM. 

Regarding high order effect, e.g. variable interaction in data, it can be captured by 
adding additional rows into hidden state matrices and additional elements into importance vectors accordingly. 
This will be the future work.




==> Exploring interpretable LSTM neural networks over multi-variable data/exp.tex <==
\section{Experiments}
\begin{table*}[htbp]
  \centering
  \caption{\small{RMSE and MAE with std. errors}}
  \small
 \resizebox{1.0\textwidth}{!}{%
  \begin{tabular}{|C{1.55cm}|C{4.0cm}|C{4.4cm}|c|}
    \hline
    % \backslashbox{Methods}
     {Dataset} &  PM2.5 & PLANT & SML  \\
    \hline
    STRX &     $52.51 \pm 0.82$, $47.35 \pm 0.92$  &  $231.43 \pm 0.19$, $193.23 \pm 0.43$ & $0.039 \pm 0.001$, $0.033 \pm 0.001$ \\
    ARIMAX &   $42.51 \pm 1.13$, $40.23 \pm 0.83$  &  $225.54 \pm 0.23$, $193.42 \pm 0.41$ & $0.060 \pm 0.002$, $0.053 \pm 0.002$ \\
    \hline
    RF &       $38.84 \pm 1.12$, $22.27 \pm 0.63$  &  $164.23 \pm 0.65$, $130.90 \pm 0.15$ & $0.045 \pm 0.001$, $0.032 \pm 0.001$ \\
    XGT &      $25.28 \pm 1.01$, $15.93 \pm 0.72$  &  $164.10 \pm 0.54$, $131.47 \pm 0.21$ & $0.017 \pm 0.001$, $0.013 \pm 0.001$ \\
    ENET &     $26.31 \pm 1.33$, $15.91 \pm 0.51$  &  $168.22 \pm 0.49$, $137.04 \pm 0.38$ & $0.018 \pm 0.001$, $0.015 \pm 0.001$ \\
    \hline
    DUAL &     $25.31 \pm 0.91$, $16.21 \pm 0.42$  & $163.29 \pm 0.54$, $130.87 \pm 0.12$ & $0.019 \pm 0.001$, $0.015 \pm 0.001$ \\
    RETAIN &   $31.12 \pm 0.97$, $20.11 \pm 0.76$   & $250.69 \pm 0.36$, $190.11 \pm 0.15$ & $0.048 \pm 0.001$, $0.037 \pm 0.001$ \\
    \hline
    IMV-Full & $24.47 \pm 0.34$, $15.23 \pm 0.61$  &  $157.32 \pm 0.21$, $128.42 \pm 0.15$  &  $0.015 \pm 0.002$, $0.012 \pm 0.001$ \\
    IMV-Tensor &  $\mathbf{24.29 \pm 0.45}$, $\mathbf{14.87 \pm 0.44}$  &  $\mathbf{156.32 \pm 0.31}$, $\mathbf{127.42 \pm 0.21}$  & $\mathbf{0.009 \pm 0.0009}$, $\mathbf{0.006 \pm 0.0005}$ \\
    \hline
\end{tabular}%
}
\vspace{-10pt}
\label{tab:full}
% \vspace{-1.5em}
\end{table*}

\subsection{Datasets}
% \footnote{https://archive.ics.uci.edu/ml/datasets.html} 
\textbf{PM2.5:}
It contains hourly PM2.5 data and the associated meteorological data in Beijing of China. PM2.5 measurement is the target series. The exogenous time series include dew point, temperature, pressure, combined wind direction, accumulated wind speed, hours of snow, and hours of rain. Totally we have $41,700$ multi-variable sequences.
% \textbf{Energy:} It collects the appliance energy use in a low energy building. The target series is the energy data logged every 10 minutes. Exogenous time series consist of $14$ variables, e.g. the house inside temperature conditions and outside weather information including temperature, wind speed, humanity and dew point from the nearest weather station.
% The number of sequence is $19,700$.
% $19,735$

% This data covers the period from July 26, 2016 to December 22, 2016, 105 days in total. 
% Each day contains 390 data points from the opening to closing of the market except that there are 210 data points on November 25 and 180 data points on December 22.
% In our experiments, we use the first 35,100 data points as the training set and the following 2,730 data points as the validation set. The last 2,730 data points are used as the test set. 
% This dataset is publicly available and will be continuously enlarged to aid the research in this direction.

\textbf{PLANT:}
This records the time series of energy production of a photo-voltaic power plant in Italy \citep{ceci2017predictive}. Exogenous data consists of 9 weather conditions variables (such as temperature, cloud coverage, etc.). The power production is the target. 
It provides 20842 sequences split into training ($70\%$), validation ($10\%$) and testing sets ($20\%$).
% Each time point is the hourly aggregation obtained as the average of all the measures available in a specified hour.

\textbf{SML} is a public dataset used for indoor temperature forecasting. 
Same as \citep{qin2017dual}, the room temperature is taken as the target series and another 16 time series are exogenous series.
The data were sampled every minute.
The first 3200, the following 400 and the last 537 data points are respectively used for training, validation, and test.
% and was smoothed with 15 minute means. 
% hourly observations.

Due to the page limitation, experimental results on additional datasets are in the supplementary material.
\begin{figure*}[htbp]
    \vskip 0.2in
    \centering
    \begin{subfigure}[t]{0.32
    \textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/var_pm-eps-converted-to.pdf}
        \caption{\small{PM2.5}}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/var_plant-eps-converted-to.pdf}
        \caption{\small{PLANT}}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/var_sml-eps-converted-to.pdf}
        \caption{\small{SML}}
    \end{subfigure}%
    ~
    \vspace{-10pt}
    \caption{\small Variable importance over epochs during the training. Top and bottom panels in each sub-figure respectively correspond to IMV-Full and IMV-Tensor. 
    In Sec. 4.4., we provide evidence from domain knowledge and show the agreement with the discoveries by IMV-Full and IMV-Tensor.
}
    \label{fig:impt_var}
    \vskip -0.2in
    %  \vspace{-15pt}
\end{figure*}

\subsection{Baselines and Evaluation Setup}
The first category of statistics baselines includes:

\textbf{STRX} is the structural time series model with exogenous variables 
~\citep{scott2014predicting, radinsky2012modeling}. 
It is consisted of unobserved components via state space models.
% and used to capture local trend variation in time series. 
% Exogenous series is incorporated through additional regression terms. 

\textbf{ARIMAX} is the auto-regressive integrated moving average with regression terms on exogenous variables~\citep{hyndman2014forecasting}. 
It is a special case of vector auto-regression in this scenario.

The second category of  machine learning baselines includes: 
% popular tree ensemble methods and regularized regression as:

\textbf{RF} refers to random forests, an ensemble learning method consisting of several decision trees~\citep{liaw2002classification} and was used in time series prediction~\citep{patel2015predicting}.
% for classification, regression and other tasks 
% It works by constructing several decision trees on various sub-samples of the dataset at training time. In the testing phase, it uses the mean prediction of the individual trees as the overall prediction to improve the predictive accuracy and control over-fitting.

\textbf{XGT} refers to the extreme gradient boosting~\citep{chen2016xgboost}. 
It is the application of boosting methods to regression trees~\citep{friedman2001greedy}. 
% GBT trains a sequence of simple regression trees and then adds together the prediction of individual trees to provide the final prediction.
% It was developed to improve the training efficiency and model performance of GBT by efficiently making use of computing resources and a more regularized model formalization. 
%is the gradient boosted tree, which 
% It has very prevailed in a variety of classification and regression predictive modeling problems.
% to control over-fitting

\textbf{ENET} represents Elastic-Net, which is a regularized regression method combining both L1 and L2 penalties of the lasso and ridge methods~\citep{zou2005regularization} and used in time series analysis~\citep{liu2010learning, bai2008forecasting}.
% \textbf{GP} stands for the Gaussian process based regression \citep{brahim2004gaussian, wu2014gaussian}, which has been successfully applied to time series. It is a supervised learning method which provides a Bayesian nonparametric approach to smoothing and interpolation.


The third category of deep learning baselines includes:

\textbf{RETAIN} uses RNNs to respectively learn weights on input data for predicting~\citep{choi2016retain}.
It defines contribution coefficients on attentions to represent feature importance. 

\textbf{DUAL} is an encoder-decoder architecture using an encoder to learn attentions and feeding pre-weighted input data into a decoder for forecasting~\citep{qin2017dual}.
It uses temporal-wise variable attentions to reflect variable importance.
% Note that temporal-wise variable attention is different from the variable-wise attention of this paper's interest.

% \textbf{cLSTM} proposes to identify Granger causal variables via sparse regularization on the weights of LSTM \citep{tank2017interpretable, tank2018neural}.
% \textbf{AttLSTM} fuses the hidden states of each variable into one hidden state via variable attention. Then it is fed into dense layers for prediction.


In ARIMAX, the orders of auto-regression and moving-average terms are set as the window size of the training data.
% via the autocorrelation and partial autocorrelation.
For RF and XGT, hyper-parameter tree depth and the number of iterations are chosen from range $[3, 10]$ and $[2, 200]$ via grid search. For XGT, L2 regularization is added by searching within $\{0.0001, 0.001, 0.01, 0.1, 1, 10\}$.
As for ENET, the coefficients for L2 and L1 penalties are selected from $\{0, 0.1, 0.3, 0.5, 0.7, 0.9, 1, 2\}$. 
For machine learning baselines, multi-variable input sequences are flattened into feature vectors. 

We implemented IMV-LSTM and deep learning baselines with Tensorflow.
% \footnote{ Code will be released upon requested.}. 
We used Adam with the mini-batch size $64$~\citep{kingma2014adam}.
For the size of recurrent and dense layers in the baselines, we conduct grid search over $\{16, 32, 64, 128, 256, 512\}$. 
The size of IMV-LSTM layers is set by the number of neurons per variable selected from $\{10, 15, 20, 25\}$.
Dropout is selected in $\{0, 0.2, 0.5\}$.
Learning rate is searched in $\{0.0005, 0.001, 0.005, 0.01, 0.05 \}$.
L2 regularization is added with the coefficient chosen from $\{0.0001, 0.001, 0.01, 0.1, 1.0\}$.
% The values that achieve the best performance over validation sets are used for evaluation.
We train each approach $5$ times and report average performance.
% and standard errors.
% To measure the effectiveness of various methods for time series prediction, 
% Among them, root mean squared error (RMSE) and mean absolute error (MAE) are two scale-dependent measures, and mean absolute percentage error (MAPE) is a scale-dependent measure.
% For baseline DUAL, we use the hyper-parameters achieving the best performance in \cite{qin2017dual}. 
% On PLANT dataset, hyper-parameters are searched in above sets of values. 
The window size (i.e. $T$) for PM2.5 and SML is set to 10 according to~\citep{qin2017dual}, while for PLANT it is 20 to test long dependency.

We consider two metrics to measure the prediction performance. RMSE is defined as $ \text{RMSE} = \sqrt[]{\sum_{k} (y_k - \hat{y}_k)^2/K} $. MAE is defined as $ \text{MAE} = \sum_{k}|y_k - \hat{y}_k|/K$.


\subsection{Prediction Performance}
% \footnote{
    % We include the detailed prediction performance analysis in the Section~\ref{subsubsec:performance_analysis} of the Appendix .
% } 
We report the prediction errors in Table~\ref{tab:full}, each cell of which presents the average RMSE and MAE with standard errors.
In particular, IMV-LSTM family outperforms baselines by around $80\%$ at most.
Deep learning baselines mostly outperform other baselines.
Boosting method XGT presents comparable performance with deep learning baselines in PLANT and SML datasets.

\textbf{Insights.} For multi-variable data carrying different patterns, properly modeling individual variables and their interaction is important for the prediction performance.
IMV-Full keeps the variable interaction in the gate updating. 
IMV-Tensor maintains variable-wise hidden states independently and only captures their interaction via the mixture attention.
Experimentally, IMV-Full and IMV-Tensor present comparable performance, though mixture on independent variable-wise hidden states in IMV-Tensor leads to the best performance.
Note that IMV-Full and IMV-Tensor are of single network structure.
Instead of composite network architectures in baselines, mixture of well-maintained variable-wise hidden states in IMV-LSTM also improves the prediction performance and empowers the interpretability shown below.
% simple attention aggregated variable-wise hidden states and prediction  
% IMV-Tensor beats baselines and IMV-Full 
% STRX and ARIMAX underperform machine learning and neural network solutions. 
% Among RF, XGT, and ENET, XGT performs the best mostly. 
% As for neural network baselines, DUAL outperforms RETAIN.
% but under-perform XGT.
% \tian{tensor, full, training time?}
% Above observations also apply to the MAE results in Table~\ref{tab:mae} and we skip the detailed description.


\subsection{Interpretation}
In this part, we qualitatively analyze the meaningfulness of variable and temporal importance.
Fig.~\ref{fig:impt_var} and Fig.~\ref{fig:impt_temp} respectively show the variable and temporal importance values during the training under the best hyper-parameters. 
The importance values learned by IMV-Full and IMV-Tensor could be slightly different, because in IMV-Tensor the gate and memory update scheme evolve independently, thereby leading to different hidden states to IMV-Full. 
IMV-LSTM is easier to understand, compared to baseline RETAIN and DUAL, since they do not show in global level importance interpretation like in Fig.~\ref{fig:impt_var} and ~\ref{fig:impt_temp}.
% As far as we know, experiments in previous work using only attentions in RNNs do not unveil the following interpretation over variable and temporal levels.
\begin{table*}[htbp]
  \centering
%   \vspace{-0.5em}
  \caption{\small{RMSE and MAE with std. errors under top $50\%$ important variables}}
  \small
%   \begin{tabular}{|C{1.5cm}|C{0.9cm}|C{0.9cm}|C{0.9cm}|}
\resizebox{1.0\textwidth}{!}{%
  \begin{tabular}{|C{1.85cm}|c|c|c|}
    \hline
     {Dataset} &  PM2.5 & PLANT & SML \\
    \hline
    DUAL &      $ 25.09 \pm 0.04$, $15.59 \pm 0.08$ &  $171.30 \pm 0.17$, $154.15 \pm 0.20$ & $0.026 \pm 0.002$, $0.018 \pm 0.002$ \\
    RETAIN &    $ 49.25 \pm 0.11$, $34.03 \pm 0.24$ & $226.38 \pm 0.72$, $167.90 \pm 0.81$  & $0.060 \pm 0.001$, $0.044 \pm 0.004$ \\
    \hline
    IMV-Full-P &  $25.14 \pm 0.54$, $ 16.01 \pm 0.52 $  &  $165.04 \pm 0.08$, $129.09 \pm 0.09$  & $0.016 \pm 0.001$,  $0.013 \pm 0.0009$ \\
    IMV-Tensor-P & $24.84 \pm 0.43$, $ 15.57 \pm 0.61$  &  $161.98 \pm 0.11$, $131.17 \pm 0.12$  & $0.013 \pm 0.0008$, $0.009 \pm 0.0005$ \\
    \hline
    IMV-Full &    $24.32 \pm 0.32$,  $15.47 \pm 0.02$     & $162.14 \pm 0.10$, $128.83 \pm 0.12$  & $0.015 \pm 0.001$, $0.011 \pm 0.002 $ \\
    IMV-Tensor &  $\mathbf{24.12 \pm 0.03}$, $\mathbf{15.10 \pm 0.01}$   & $\mathbf{157.64 \pm 0.14}$, $\mathbf{128.16 \pm 0.13}$ & $\mathbf{0.007 \pm 0.0005}$, $\mathbf{0.006 \pm 0.0003}$ \\
    \hline
\end{tabular}%
}
\vspace{-10pt}
\label{tab:top50}
% \vspace{-1.5em}
\end{table*}

\textbf{Variable importance.}
In Fig.~\ref{fig:impt_var}, top and bottom panels in each sub-fig show the variable importance values w.r.t. training epochs from IMV-Full and IMV-Tensor. Overall, variable importance values converge during the training and the ranking of variable importance is identified at the end of the training.
Variables with high importance values contribute more to the prediction of IMV-LSTM.

In Fig.~\ref{fig:impt_var}(a), for PM2.5 dataset, variables ``Wind speed'', ``Pressure'', ``Snow'', ``Rain'' are high ranked by IMV-LSTM. 
According to a recent work studying air pollution~\citep{liang2015assessing}, ``Dew Point'' and ``Pressure'' are both related to PM2.5 and they are also inter-correlated. 
% In prediction task, subset of correlated variables could provide sufficient prediction power. 
One ``Pressure'' variable is enough to learn accurate forecasting and thus has the high importance value.
Strong wind can bring dry and fresh air.
``Snow'' and ``Rain'' amount are related to the air quality as well.
Variables important for IMV-LSTM are in line with the domain knowledge in \citep{liang2015assessing}.

Fig.~\ref{fig:impt_var}(b) shows that in PLANT dataset in addition to ``Irradiance'' and  ``Cloud cover'', ``Wind speed'', ``Humidity'' as well as ``Temperature'' are also high ranked and relatively used more in IMV-LSTM to provide accurate forecasting. 
As is discussed in \citep{mekhilef2012effect, ghazi2014effect}, humidity causes dust deposition and consequentially degradation in solar cell efficiency. Increased wind can move heat from the cell surface, which leads to better efficiency.

Fig.~\ref{fig:impt_var}(c) demonstrates that variables ``Humid. room'', ``CO2 room'', and ``Lighting room''
% 'Temp. dinning', 'Humid. dinning', 'Lighting dinning', 'Sunlight in east', 'Sunlight in west' 
are relatively more important for IMV-LSTM (``Humid.'' represents humidity). 
As is suggested in~\citep{nguyen2014relationship, hoppe1993indoor}, humidity is correlated to the indoor temperature.

\textbf{Temporal importance.}
Fig.~\ref{fig:impt_temp} demonstrate the temporal importance values of each variable at the ending of the training.
The lighter the color, the more the corresponding data contributes to the prediction.

Specifically, in Fig.~\ref{fig:impt_temp}(a), short history of variables ``Snow'' and ``Wind speed'' contributes more to the prediction. PM2.5 itself has relatively long-term auto-correlation, i.e. around $5$ hours.   
Fig.~\ref{fig:impt_temp}(b) shows that recent data of aforementioned important variables ``Wind'' and ``Temperature'' are highly used for prediction, while ``Cloud-cover'' is long-term correlated to the target, i.e. around $13$ hours.
In Fig.~\ref{fig:impt_temp}(c) temporal importance values are mostly uniform, though ``Humid. dinning'' has short correlation, ``Outdoor temp.'' and ``Lighting dinning'' are relatively long-term correlated to the target.
\vspace{-0.17cm}
\begin{figure}[!ht]
    \centering
    \begin{subfigure}[]{0.45\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/var_temp_pm-eps-converted-to.pdf}
        \caption{\small{PM2.5}}
    \end{subfigure}
    ~
    \begin{subfigure}[]{0.45\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/var_temp_plant-eps-converted-to.pdf}
        \caption{\small{PLANT}}
    \end{subfigure}
    ~
    \begin{subfigure}[]{0.45\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/var_temp_sml-eps-converted-to.pdf}
        \caption{\small{SML}}
    \end{subfigure}
    ~
    \vspace{-10pt}
    \caption{\small Variable-wise temporal importance interpretation. Left and right panels respectively correspond to IMV-Full and IMV-Tensor. Different patterns of decays in the temporal importance of variables are observed, which brings the additional interpretation of the dynamics of each variable. (Best viewed in color)}
    \vspace{-15pt}
    \label{fig:impt_temp}
\end{figure}
% \setlength{\belowcaptionskip}{-35pt}

\subsection{Variable Selection}
In this group of experiments, we quantitatively evaluate the efficacy of variable importance through the lens of prediction tasks.
We focus on IMV-LSTM family and RNN baselines, i.e. DUAL and RETAIN.

Specifically, for each approach, we first rank variables respectively according to the variable importance in IMV-LSTM, variable attention in DUAL and contribution coefficients in RETAIN.
Meanwhile, we add one more group of baselines denoted by IMV-Full-P and IMV-Tensor-P. 
The label ``-P'' represents that the Pearson correlation is used to rank the variables with the highest (absolute) correlation values to the target and the selected data is fed to IMV-LSTM.

Then we rebuild datasets only consisting of top $50\%$ ranked variables by respective methods, retrain each model with these new datasets and obtain the errors in Table~\ref{tab:top50}.

\textbf{Insights.}
Ideally, effective variable selection enables the corresponding retrained models to have comparable errors in comparison to their counterparts trained on full data in Table~\ref{tab:full}.
IMV-Full and IMV-Tensor present comparable and even lower errors in Table~\ref{tab:top50}, while DUAL and RETAIN have higher errors mostly. 
Pearson correlation measures linear relation. Selecting variables based on it neglects non-linear correlation and is not suitable for LSTM to attain the best performance.
An additional advantage of variable selection is the training efficiency, e.g. training time of each epoch in IMV-Tensor is reduced from $\sim$16 to $\sim$11 sec.

==> Exploring interpretable LSTM neural networks over multi-variable data/intro.tex <==
\section{Introduction}

Recently, recurrent neural networks (RNNs), especially long short-term memory (LSTM)~\citep{hochreiter1997long} and gated recurrent units (GRU)~\citep{cho2014properties}, have been proven to be powerful sequence modeling tools in various tasks e.g. language modelling, machine translation, health informatics, time series, and speech~\citep{ke2018focused, lin2017hybrid, guo2016robust, lipton2015learning, sutskever2014sequence, bahdanau2014neural}.
In this paper, we focus on RNNs over multi-variable time series consisting of target and exogenous variables.
% Each variable corresponds to a monitoring over .
RNNs trained over such multi-variable data capture nonlinear correlation of historical values of target and exogenous variables to the future target values. 

In addition to forecasting, interpretable RNNs are desirable for gaining insights into the important part of data for RNNs achieving good prediction performance~\citep{hu2018listening, foerster2017input, lipton2016mythos}.
In this paper, we focus on two types of importance interpretation: variable importance and variable-wise temporal importance.
First, in RNNs variables differ in predictive power on the target, thereby contributing differently to the prediction~\citep{feng2018nonparametric, riemer2016correcting}.
Second, variables also present different temporal relevance to the target one ~\citep{kirchgassner2012introduction}.
For instance, for a variable instantaneously correlated to the target, its short historical data contributes more to the prediction. 
The ability to acquire this knowledge enables additional applications, e.g. variable selection. 

% Our daily life is now surrounded by various types of sensors, ranging from smart phones, video cameras, Internet of things, to robots. The observations yield by such devices over time are naturally organized in time series data~\citep{qin2017dual, yang2015deep}.

%  --- reference list: interpretability
% \citep{hu2018listening, siggiridou2016granger, zhou2015probabilistic}.
% \citep{foerster2017input}.
% tsang2017detecting

%Regarding the benefit of variable importance, we could use statistical regression as an analogy. 

%In many studies, regression analysis not only serves for predicting but also for identifying the relevance between variables and the target. It has a set of associated tools to interpret the learned regression model. For instance, in the renewable energy research area, by analyzing the weights and significances of linear regression, researchers can understand which variable is strongly correlated to the target [1]. 

%On the contrary, when RNN or LSTM is used to model multi-variable series, there are few associated tools to quantify and identify the different strength of variable relatedness. This paper aims to fill this gap. Meanwhile, as is shown in the experiments, learned variable importance bring additional benefits, e.g. removing redundant data via importance ranking, improving the predicting performance as well as the training efficiency. 


% exogenous variables have different contribution w.r.t. the prediction of the target one
% Each of these sources may have a different
% bias and noise with respect to the original signal that needs
% to be recovered (cf. time series in Figure 1). Moreover, these
% sources are usually strongly correlated and lead-lag relationships
% are possible (e.g. a market-maker with more clients
% can update its view more frequently and precisely than one
% with fewer clients). Therefore, the significance of each of
% the available past observations might be dependent on some
% other factors that can change in time

% ---- reference list
% castAtt2018
% Autoregressive Convolutional Neural Networks for Asynchronous Time Series

However, current RNNs fall short of the aforementioned interpretability for multi-variable data due to their opaque hidden states.
Specifically, when fed with the multi-variable observations of the target and exogenous variables, RNNs blindly blend the information of all variables into the hidden states used for prediction.
It is intractable to distinguish the contribution of individual variables into the prediction through the sequence of hidden states~\citep{zhang2017stock}. 

Meanwhile, individual variables typically present different dynamics. 
This information is implicitly neglected by the hidden states mixing multi-variable data, thereby potentially hindering the prediction performance.
% This is because when multiple driving (exogenous) series are available, the network cannot explicitly select relevant driving series to make predictions. In addition, they have mainly been used for classification, rather than time series prediction.
% cinar2017position


Existing works aiming to enhance the interpretability of recurrent neural networks rarely touch the internal structure of RNNs to overcome the opacity of hidden states on multi-variable data. 
They still fall short of aforementioned two types of interpretation~\citep{montavon2018methods, foerster2017input, che2016interpretable}. 
% Much effort has been made to enhance the interpretability of recurrent neural networks~\citep{montavon2018methods, foerster2017input, che2016interpretable}.
One category of the approaches is to perform post-analyzing on trained RNNs by perturbation on training data or gradient based methods~\citep{ancona2018towards, ribeiro2018anchors, lundberg2017unified, shrikumar2017learning}.
Another category is to build attention mechanism on hidden states of RNNs to characterize the importance of different time steps~\citep{qin2017dual, choi2016retain}.

% bahdanau2014neural
% chorowski2015attention
% vaswani2017attention, vinyals2015pointer

% attention-based neural networks have been proposed to enhance the ability of RNN in selectively using long-term memory and the interpretability
% Nevertheless, current attention mechanism is mostly applied to hidden states across time steps and capture globally temporal information, thereby failing to uncover fine-grained variable level importance.

In this paper we aim to achieve a unified framework of accurate forecasting and importance interpretation.
In particular, the contribution is fourfold:
% First, by using hidden matrix and specialized update scheme, LSTM is enabled to capture individiual variable's dyanmics, which will facilitate the prediction and interpretation. 
% In this paper, this family of interpretable multi-variable LSTM is denoted by IMV-LSTM.  
% Second, we develop a novel mixture attention mechanism to summarize variable-wise hidden states.
% Third, we develop the training process based on probabilistic mixture attention to learn network parameter, temporal and variable importance measures simultaneously with theoretical upper bound. 
% Lastly, we perform extensive experimental evaluation of IMV-LSTM against statistical, machine learning and deep learning based baselines to demonstrate the superior prediction performance and interpretability of IMV-LSTM.
% The idea of IMV-LSTM easily applies to other RNN structures, e.g. GRU and stacked recurrent layers. This will be the future work.
\begin{itemize}
\item We explore the structure of LSTM to enable variable-wise hidden states capturing individual variable's dynamics. 
It facilitates the prediction and interpretation.
This family of LSTM is referred to as \textbf{I}nterpretable \textbf{M}ulti-\textbf{V}ariable LSTM, i.e. IMV-LSTM.
\item A novel mixture attention mechanism is designed to summarize variable-wise hidden states and model the generative process of the target.
\item We develop a training method based on probabilistic mixture attention to learn network parameter, variable and temporal importance measures simultaneously.
\item Extensive experimental evaluation of IMV-LSTM against statistical, machine learning and deep learning based baselines demonstrate the superior prediction performance and interpretability of IMV-LSTM.
The idea of IMV-LSTM easily applies to other RNN structures, e.g. GRU and stacked recurrent layers. 
% This will be the future work.
\end{itemize}


% --- interpretability

% The Nonlinear autoregressive exogenous (NARX)
% model, which predicts the current value of a time
% series based upon its previous values as well as the

% But, the gain in accuracy from use of RNNs is at the cost of model output that is notoriously difficult to interpret. 

% --- attention
% The key idea of the attention mechanism is to perform prediction by using weighted sum of hidden states across all the time steps. The weights dependent on the hidden states provide explicit interpretation about the importance of previous steps w.r.t. the predicted step. 
% introduce extra source of information to guide the extraction of sentence
% Recently, a hierarchical attention network [Yang et al., 2016], which uses two layers of attention mechanism to select relevant encoder hidden states across all the time steps, was also developed.
% self-attention mechanism allows extracting different aspects

% Time series, a sequence of observations over time, is being generated in a wide variety of areas \citep{qin2017dual, lin2017hybrid}.
% Predicting future values of time series has been widely applied in many areas.

% e.g., financial market prediction [Wu et al., 2013], 
% weather forecasting [Chakraborty et al., 2012], and 
% complex dynamical system analysis [Liu and Hauskrecht, 2015]. 
% Recently, neural networks have been proven to be dramatical powerful in a wide spectrum of domains, e.g., natural language processing, computer vision, speech recognition, time series analysis, etc~\citep{wang2016morphological,sutskever2014sequence,yang2015deep,lipton2015learning,guo2016robust}. 
% A class of neural network architecture called Recurrent Neural Networks (RNN) is specifically designed to model sequential data. 
% Traditional RNNs suffer from the problem of vanishing gradients~\citep{bengio1994learning} and thus have difficulty in capturing long-term dependencies. 
% Among variants of RNN, 

% The Recurrent layers with GRU [6] and LSTM [15] unit are carefully designed to memorize the historical information and hence to be aware of relatively long-term dependencies.
% they cannot model nonlinear relationships and do not differentiate among the exogenous (driving) input terms.

% In many settings, data is collected as multiple time series, where each recorded time series is an observation of some underlying dynamical process of interest. These observations are often time-marked with known event times, and one desires to do a range of standard analyse
% the values of the target series by using autoregressive part itself and exogenous series

==> Exploring interpretable LSTM neural networks over multi-variable data/model.tex <==
\section{Interpretable Multi-Variable LSTM}\label{sec:mv}
In the following we will first explore the internal structure of LSTM to enable hidden states to encode individual variables, such that the contribution from individual variables to the prediction can be distinguished.
Then, mixture attention is designed to summarize these variable-wise hidden states for predicting. 
The described method can be easily extended to multi-step ahead prediction via iterative methods as well as vector regression~\citep{deepmulti2018, cheng2006multistep}.
\begin{figure*}[htbp!]
% \centering
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width = 0.9\textwidth]{figures/archi-eps-converted-to.pdf}}
\caption{A toy example of a IMV-LSTM with a two-variable input sequence and the hidden matrix of  $4$-dimensions per variable.
Circles represent one dimensional elements.
Purple and blue colors correspond to two variables. 
Blocks containing rectangles with circles inside represent input data and hidden matrix.
Panel (a) exhibits the derivation of hidden update $\mathbf{\tilde{j}}_t$. 
Grey areas represent transition weights. 
Panel (b) demonstrates the mixture attention process. (best viewed in color)}
\label{fig:graph}
\end{center}
\vskip -0.2in
\end{figure*}

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
% \caption{Historical locations and number of accepted papers for International
% Machine Learning Conferences (ICML 1993 -- ICML 2008) and International
% Workshops on Machine Learning (ML 1988 -- ML 1992). At the time this figure was
% produced, the number of accepted papers for ICML 2008 was unknown and instead
% estimated.}
% \label{icml-historical}
% \end{center}
% \vskip -0.2in
% \end{figure}

Assume we have $N$-$1$ exogenous time series and a target series $\mathbf{y}$ of length $T$, where $\mathbf{y} = [ y_1, \cdots, y_T ]$ and $\mathbf{y} \in \mathbb{R}^T$. 
{Vectors are assumed to be in column form throughout this paper.}
By stacking exogenous time series and target series, we define a multi-variable input series as
$\mathbf{X}_{T} = \{ \mathbf{x}_1, \cdots, \mathbf{x}_T  \}$, 
where $\mathbf{x}_t = [ \mathbf{x}_{t}^1, \cdots, \mathbf{x}_{t}^{N-1}, {y}_{t} ]$.
Both of $\mathbf{x}_{t}^{n}$ and ${y}_{t}$ can be multi-dimensional vector.
% , and we simplify the presentation below for one dimension.
% For simplicity, we assume they are one dimensional. 
$\mathbf{x}_t \in \mathbb{R}^N$ is the multi-variable input at time step $t$.
% and $x_{t}^n \in \mathbb{R}$ is the observation of $n$-th exogenous time series at time $t$.
% each dimension corresponds to the observations of a variable. since each hidden state ingest information from all input variable, has to develop seperated rnn to individual model 
It is also free for $\mathbf{X}_T$ to merely include exogenous variables, which does not affect the methods presented below. 

Given $\mathbf{X}_T$, we aim to learn a non-linear mapping to predict the next values of the target series, namely $\hat{y}_{T+1} = \mathcal{F}(\mathbf{X}_T)$.

Meanwhile, the other desirable byproduct of learning $\mathcal{F}(\mathbf{X}_T)$ is the variable and temporal importance measures.
Mathematically, we aim to derive variable importance vector $\mathbf{I} \in R^{N}_{\geq 0}$, $\sum_{n=1}^N \text{I}_{n} = 1$ and variable-wise temporal importance vector $\mathbf{T}^n \in R^{T-1}_{\geq 0}$ (w.r.t. variable $n$), $\sum_{k = 1}^{T-1} \text{T}^n_{k} = 1$.
Elements of these vectors are normalized (i.e. sum to one) and reflect the relative importance of the corresponding variable or time instant w.r.t. the prediction.

\subsection{Network Architecture}
The idea of IMV-LSTM is to make use of hidden state matrix and to develop associated update scheme, such that each element (e.g. row) of the hidden matrix encapsulates information exclusively from a certain variable of the input.

To distinguish from the hidden state and gate vectors in a standard LSTM, hidden state and gate matrices in IMV-LSTM are denoted with tildes.
Specifically, we define the hidden state matrix at time step $t$ as $\mathbf{\tilde{h}}_t = [ \mathbf{h}_t^{1} \, , \cdots, \, \mathbf{h}_t^{N} ]^\top$, where $\mathbf{\tilde{h}}_t \in \mathbb{R}^{N \times d}$, $\mathbf{h}_t^{n} \in \mathbb{R}^{d}$.
The overall size of the layer is derived as $D = N \cdot d$. 
The element $\mathbf{h}_t^{n}$ of $\mathbf{\tilde{h}}_t$ is the hidden state vector specific to $n$-th input variable.

Then, we define the input-to-hidden transition as $\boldsymbol{\mathcal{U}}_j = [\mathbf{U}^{1}_j \, , \cdots, \, \mathbf{U}^{N}_j ]^\top$, 
where $\boldsymbol{\mathcal{U}}_j \in \mathbb{R}^{N \times d \times d_0 }$, $\mathbf{U}^{n}_j \in \mathbb{R}^{d \times d_0} $ and $d_0$ is the dimension of individual variables at each time step.
The hidden-to-hidden transition is defined as: 
$\boldsymbol{\mathcal{W}}_j = [ \mathbf{W}_j^{1} \, \cdots \, \mathbf{W}_j^{N} ]$, 
where $\boldsymbol{\mathcal{W}}_j \in \mathbb{R}^{N \times d \times d}$ and 
$\mathbf{W}_j^{n} \in \mathbb{R}^{d \times d}$.
% Such transition tensors enable recurrent transition functions specific for each input variable.

As standard LSTM neural networks~\citep{hochreiter1997long}, IMV-LSTM has the input $\mathbf{i}_t$, forget $\mathbf{f}_t$, output gates $\mathbf{o}_t$ and the memory cells $\mathbf{c}_t$ in the update process.
Given the newly incoming input $\mathbf{x}_t$ at time $t$ and the hidden state matrix $\mathbf{\tilde{h}}_{t-1}$, the hidden state update is defined as:
\begin{equation}
\mathbf{\tilde{j}}_t = \tanh \left( \boldsymbol{\mathcal{W}}_j \circledast \mathbf{\tilde{h}}_{t-1} + \boldsymbol{\mathcal{U}}_j \circledast \mathbf{x}_t + \mathbf{b}_j \right) \,,  \label{eq:j}
\end{equation}
where $\mathbf{\tilde{j}}_t = [ \, \mathbf{j}_t^1, \cdots, \mathbf{j}_t^N \, ]^{\top}$ has the same shape as hidden state matrix $\mathbb{R}^{N \times d}$. 
Each element $ \mathbf{j}_t^n \in \mathbb{R}^{d}$ corresponds to the update of the hidden state
w.r.t. input variable $n$. Term $\boldsymbol{\mathcal{W}}_j \circledast \mathbf{\tilde{h}}_{t-1}$ and $\boldsymbol{\mathcal{U}}_j \circledast \mathbf{x}_t $ respectively capture the update from the hidden states at the previous step and the new input.
The tensor-dot operation $\circledast$ is defined as the product of two tensors along the $N$ axis,
e.g., $\boldsymbol{\mathcal{W}}_j \circledast \mathbf{\tilde{h}}_{t-1} = [ \mathbf{W}_j^1 \mathbf{h}_{t-1}^1 \, , \cdots, \, \mathbf{W}_j^N \mathbf{h}_{t-1}^N ]^\top $ where $ \mathbf{W}_j^n \mathbf{h}_{t-1}^n  \in \mathbb{R}^{d}$.

% Define the tensor-dot operation $\circledast$ as the product of two tensors along the $N$ axis. 
% For instance, 
% % the tensor-dot of $\boldsymbol{\mathcal{W}}_j$ and $\mathbf{\tilde{h}}_{t-1}$ along the axis $N$ is expressed as 
% $\boldsymbol{\mathcal{W}}_j \circledast \mathbf{\tilde{h}}_{t-1} = [ \mathbf{W}_j^1 \mathbf{h}_{t-1}^1 \, , \cdots, \, \mathbf{W}_j^N \mathbf{h}_{t-1}^N ]^\top $, where $ \mathbf{W}_j^n \mathbf{h}_{t-1}^n  \in \mathbb{R}^{d}$.

Depending on different update schemes of gates and memory cells,  we proposed two realizations of IMV-LSTM, i.e. IMV-Full in Equation set \ref{eqset:1} and IMV-Tensor in Equation set \ref{eqset:2}.
In these two sets of equations, $\text{vec}(\cdot)$ refers to the vectorization operation, which concatenates columns of a matrix into a vector.
The concatenation operation is denoted by $\oplus$ and element-wise multiplication is denoted by $\odot$.
Operator $\text{matricization}(\cdot)$ reshapes a vector of $\mathbb{R}^D$ into a matrix of $\mathbb{R}^{N \times d}$.
\begin{minipage}{0.47\textwidth}
\begin{align}
&\begin{bmatrix}
        \mathbf{i}_t \\
        \mathbf{f}_t \\
        \mathbf{o}_t 
        \end{bmatrix} =  \sigma \left( \mathbf{W} \text{ } [\mathbf{x}_t \oplus \text{vec}(\text{ } \mathbf{\tilde{h}}_{t-1})] + \mathbf{b} \right) \label{eq:full_gate}\\
&\text{ }\mathbf{c}_t = \mathbf{f}_t \odot \mathbf{c}_{t-1} + \mathbf{i}_t \odot \text{vec}( \text{ }\mathbf{\tilde{j}}_t) \label{eq:full_c}\\
&\text{ }\mathbf{\tilde{h}}_t = \text{matricization}( \mathbf{o}_t \odot \tanh(\mathbf{c}_t) ) \label{eq:full_h}
\end{align}
\equationset{IMV-Full}\label{eqset:1}
\end{minipage}%
%\hfill\vline
\hfill
\begin{minipage}{0.47\textwidth}
\begin{align}
&\begin{bmatrix}
        \mathbf{\tilde{i}}_t \\
        \mathbf{\tilde{f}}_t \\
        \mathbf{\tilde{o}}_t 
        \end{bmatrix} =  \sigma \left( \boldsymbol{\mathcal{W}} \circledast \mathbf{\tilde{h}}_{t-1} + \boldsymbol{\mathcal{U}} \circledast \mathbf{x}_t + \mathbf{b} \right) \label{eq:tensor_gate}\\
&\text{ }\mathbf{\tilde{c}}_t = \mathbf{\tilde{f}}_t \odot \mathbf{\tilde{c}}_{t-1} + \mathbf{\tilde{i}}_t \odot \mathbf{\tilde{j}}_t \label{eq:tensor_c}\\
&\text{ }\mathbf{\tilde{h}}_t = \mathbf{\tilde{o}}_t \odot \tanh(\mathbf{\tilde{c}}_t) \label{eq:tensor_h}
\end{align}
\equationset{IMV-Tensor}\label{eqset:2}
\end{minipage}

\textbf{IMV-Full}: 
With vectorization in Eq.~\eqref{eq:full_gate} and \eqref{eq:full_c}, IMV-Full updates gates and memories using full $\mathbf{\tilde{h}_{t-1}}$ and $\mathbf{\tilde{j}_t}$ regardless of the variable-wise data in them. 
By simple replacement of the hidden update in standard LSTM by $\mathbf{\tilde{j}}_t$, IMV-Full behaves identically to standard LSTM while enjoying the interpretability shown below.

\textbf{IMV-Tensor}:
By applying tensor-dot operations in Eq.~\eqref{eq:tensor_gate}, gates and memory cells are matrices as well, elements of which have the correspondence to input variables as hidden state matrix $\mathbf{\tilde{h}}_t$ does.
$\boldsymbol{\mathcal{W}}$ and $\boldsymbol{\mathcal{U}}$ have the same shapes as $\boldsymbol{\mathcal{W}_j}$ and $\boldsymbol{\mathcal{U}_j}$ in Eq.~\eqref{eq:j}.
% \tian{relation to lstm, proof: variable-wise hidden, equivalence, attention aggregation}

In IMV-Full and IMV-Tensor, gates only scale $\mathbf{\tilde{j}_t}$ and $\mathbf{\tilde{c}}_{t-1}$ and thus retain the variable-wise data organization in $\mathbf{\tilde{h}}_t$. 
Meanwhile, based on tensorized hidden state Eq.~\eqref{eq:j} and gate update Eq.~\eqref{eq:tensor_gate}, IMV-Tensor can also be considered as a set of parallel LSTMs, each of which processes one variable series and then merges via the mixture. 
The derived hidden states specific to each variable are aggregated on both temporal and variable level through the mixture attention.

Next, we provide the analysis about the complexity of IMV-LSTM through Lemma~\ref{lemma:size} and Lemma~\ref{lemma:time}.

\begin{lemma}\label{lemma:size}
	Given time series of $N$ variables, assume a standard LSTM and IMV-LSTM layer both have size $D$, i.e. $D$ neurons in the layer.
	Then, compared to the number of parameters of the standard LSTM, IMV-Full and IMV-Tensor respectively reduce the network complexity by $(N-1)D + (1-1/N)D \cdot D$ and $4(N-1)D + 4(1-1/N)D \cdot D$ number of parameters. 
\end{lemma}
\begin{proof}
	In a standard LSTM of layer size $D$, trainable parameters lie in the hidden and gate update functions.
	In total, these update functions have $4 D\cdot D + 4 N \cdot D + 4 D$ parameters, where $4 D\cdot D + 4 N \cdot D$ comes from the transition and $4D$ corresponds to the bias terms.	
	For IMV-Full, assume each input variable corresponds to one-dimensional time series. 
	Based on Eq.~\ref{eq:j}, the hidden update has $2D + D^2/N$ trainable parameters. 
	Equation set \ref{eqset:1} gives rise to the number of parameters equal to that of the standard LSTM.
	Therefore, the reduce number of parameters is $(N-1)D + (1-1/N)D \cdot D$.
	As for IMV-Tensor, more parameter reduction stems from that the gate update functions in Equation set \ref{eqset:2} make use of the tensor-dot operation as Eq.~\ref{eq:j}. 
% 	Likewise, the reduced amount of parameters can be derived.   
\end{proof}

\begin{lemma}\label{lemma:time}
	For time series of $N$ variables and the recurrent layer of size $D$, IMV-Full and IMV-Tensor respectively have the computation complexity at each update step as: $\mathcal{O}(D^2 + N\cdot D)$ and $\mathcal{O}(D^2/N + D)$.
\end{lemma}
\begin{proof}
Assume that $D$ neurons of the recurrent layer in IMV-Full and IMV-Tensor are evenly assigned to $N$ input variables, namely each input variable has $d = D/N$ corresponding neurons. 
For IMV-Full, based on Eq.~\ref{eq:j}, the hidden update has computation complexity $N \cdot d^2 + N \cdot d$, while the gate update process has the complexity $D^2 + N \cdot D$. Overall, the computation complexity is $\mathcal{O}(D^2 + N\cdot D)$, which is identical to the complexity of a standard LSTM.
As for IMV-Tensor, since the gate update functions in Equation set \ref{eqset:2} make use of the tensor-dot operation as Eq.~\ref{eq:j}, gate update functions have the same computation complexity as Eq.~\ref{eq:j}. The overall complexity is $\mathcal{O}(D^2/N + D)$, which is $1/N$ of the complexity of a standard LSTM. 
\end{proof}

Basically, Lemma~\ref{lemma:size} and Lemma~\ref{lemma:time} indicate that a high number of input variables leads to a large portion of parameter and computation reduction in IMV-LSTM family.

\subsection{Mixture Attention}
After feeding a sequence of $\{ \mathbf{x}_1, \cdots, \mathbf{x}_T \}$ into IMV-Full or IMV-Tensor, we obtain a sequence of hidden state matrices $\{ \mathbf{\tilde{h}}_1, \cdots, \mathbf{\tilde{h}}_{T} \}$, where the sequence of hidden states specific to variable $n$ is extracted as $\{ \mathbf{h}_1^n, \cdots, \mathbf{h}_T^n \}$. 

The idea of mixture attention mechanism as follows.
Temporal attention is first applied to the sequence of hidden states corresponding to each variable, so as to obtain the summarized history of each variable. 
Then by using the history enriched hidden state of each variable, variable attention is derived to merge variable-wise states. 
These two steps are assembled into a probabilistic mixture model~\citep{zong2018deep, graves2013generating, bishop1994mixture}, which facilitates the subsequent learning, predicting, and interpreting.  

In particular, the mixture attention is formulated as:
% our attention mechanism is based on a probabilistic mixture of experts model \citep{zong2018deep, graves2013generating, shazeer2017outrageously} over $y_{T+1}$ as:
% \begin{equation}\label{eq:mix}
\begin{align}\label{eq:mix}
& p(y_{T+1} \, | \mathbf{X}_{T}) \nonumber  \\ 
& = \sum_{n=1}^{N} p(y_{T+1} | z_{T+1} = n, \mathbf{X}_{T} ) \cdot \Pr(z_{T+1} = n | \mathbf{X}_{T}) \nonumber \\
& =  \sum_{n=1}^{N} p(y_{T+1} \, | \, z_{T+1} = n, \mathbf{h}_1^n, \cdots, \mathbf{h}_T^n ) \nonumber \\ 
&\quad \cdot \Pr(z_{T+1} = n \, | \, \mathbf{\tilde{h}}_1, \cdots, \mathbf{\tilde{h}}_{T}) \nonumber \\
& =  \sum_{n=1}^{N} p( y_{T+1} \, | \, z_{T+1} = n, \underbrace{\mathbf{h}_T^n \oplus \mathbf{g}^n}_{ {\substack{\text{variable-wise} \\ \text{temporal attention}}}} ) \\ 
&\quad \cdot \underbrace{ \Pr(z_{T+1} = n \, | \, \mathbf{h}_T^1 \oplus \mathbf{g}^1, \cdots, \mathbf{h}_T^N \oplus \mathbf{g}^N )}_{\text{Variable attention}} \nonumber  
\end{align}
In Eq. \eqref{eq:mix}, we introduce a latent random variable $z_{T+1}$ into the the density function of $y_{T+1}$ to govern the generation process.
$z_{T+1}$ is a discrete variable over the set of values $\{ 1, \cdots, N \}$ corresponding to $N$ input variables.
Mathematically, $p( y_{T+1} \, | \, z_{T+1} = n, \mathbf{h}_T^n \oplus \mathbf{g}^n )$ characterizes the density of $y_{T+1}$ conditioned on historical data of variable $n$, while the prior of $z_{T+1}$, i.e. $\Pr(z_{T+1} = n \, | \, \mathbf{h}_T^1 \oplus \mathbf{g}^1, \cdots, \mathbf{h}_T^N \oplus \mathbf{g}^N )$ controls to what extent $y_{T+1}$ is driven by variable $n$.

Context vector $\mathbf{g}^n$ is computed as the temporal attention weighted sum of hidden states of variable $n$, i.e., $\mathbf{g}^n = \sum_t \alpha_t^n \mathbf{h}_t^n$. The attention weight $\alpha_t^n$ is evaluated as $\alpha_t^n = \frac{\exp{( \, \text{f}_n(\mathbf{h}_t^n)} \,)}{ \sum_k \exp{( \, \text{f}_n(\mathbf{h}_k^n)} \,) }$,
% \begin{equation}
% \alpha_t^n = \frac{\exp{( \, \text{f}_n(\mathbf{h}_t^n)} \,)}{ \sum_k \exp{( \, \text{f}_n(\mathbf{h}_k^n)} \,) } \,,
% \end{equation}
where $\text{f}_n(\cdot)$ can be a flexible function specific to variable $n$, e.g. neural networks.
% ~\citep{bahdanau2014neural}.

For $p( y_{T+1} \, | \, z_{T+1} = n, \mathbf{h}_T^n \oplus \mathbf{g}^n )$, 
without loss of generality, we use a Gaussian output distribution parameterized by $[\, \mu_n, \sigma_n] = \varphi_n(\, \mathbf{h}_T^n \oplus \mathbf{g}^n )$, where $\varphi_n(\cdot)$ can be a feed-forward neural network.
It is free to use other distributions.

% \begin{equation}
% p( y_{T+1} \, | \, z_{T+1} = n, \mathbf{h}_T^n \oplus \mathbf{g}^n ) = \mathcal{N}( y_{T+1} | \, \mu_n, \sigma_n )
% \end{equation}
% \tao{Eq. 10 appears without description and connection.}

$\Pr(z_{T+1} = n \, | \, \mathbf{h}_T^1 \oplus \mathbf{g}^1, \cdots, \mathbf{h}_T^N \oplus \mathbf{g}^N )$ is derived by a softmax function over $\{ \text{f}( \, \mathbf{h}_T^n \oplus \mathbf{g}^n ) \}_N$, where $\text{f}(\cdot)$ can be a feedforward neural network shared by all variables. 

% \tao{feel like it could be more clear if we organize the text by $p( y_{T+1} \, | \, z_{T+1} = n, \mathbf{h}_T^n \oplus \mathbf{g}^n )$ and $\Pr(z_{T+1} = n \, | \, \mathbf{h}_T^1 \oplus \mathbf{g}^1, \cdots, \mathbf{h}_T^N \oplus \mathbf{g}^N )$. currently, they are combined together.}

\subsection{Learning to Interpret and Predict}
In the learning phase, the set of parameters in the neural network and mixture attention is denoted by $\Theta$.
Given a set of $M$ training sequences $\{\mathbf{X}_{T}\}_M$ and $\{y_{T+1}\}_M$, we aim to learn both $\Theta$ and importance vectors $\mathbf{I}$ and $\{\mathbf{T}^n\}_N$ for prediction and insights into the data.

Next, we first illustrate the burden of directly interpreting attention values and then present the training method combining parameter and importance vector learning, without the need of post analyzing. 

Importance vectors $\mathbf{I}$ and $\{\mathbf{T}^n\}_N$ reflect the global relations in variables, while the attention values derived above are specific to data instances.
Moreover, it is nontrivial to decipher variable and temporal importance from attentions.

For instance, during the training on PLANT dataset used in the experiment section, we collect variable and variable-wise temporal attention values of training instances.
In Fig~\ref{fig:att_interpret}, left panels plots the histograms of variable attention of three variables in PLANT at two different epochs.
It is difficult to fully discriminate variable importance from these histograms.
Likewise, in the right panel, histograms of temporal attentions at certain time lags of variable ``P-temperature'' at two different epochs does not ease the importance interpretation.
Time lag represents the look-back time step w.r..t the current one.
Similar phenomena are observed in other variables and datasets during the experiments.

In the following, we develop the training procedure based on the Expectation–Maximization (EM) framework for the probabilistic model with latent variables, i.e. Eq.~\eqref{eq:mix} in this paper. 
Index $m$ in the following corresponds to the training data instance. 
It is omitted in $\mathbf{h}_T^n$ and $\mathbf{g}^n$ for simplicity.

The loss function to minimize is derived as:
\begin{equation}\label{eq:loss}
\textstyle
\begin{split}
& \mathcal{L}(\Theta, \mathbf{I} ) = \\
&\quad - \sum_{m=1}^{M}  \mathbb{E}_{q_m^n}[ \, \log p( y_{T+1, m} \, | \, z_{T+1, m} = n, \mathbf{h}_T^n \oplus \mathbf{g}^n ) ] \\
&\quad - \mathbb{E}_{q_m^n}[ \, \log \Pr(z_{T+1, m} = n \, | \, \mathbf{h}_T^1 \oplus \mathbf{g}^1, \cdots, \mathbf{h}_T^N \oplus \mathbf{g}^N )] \\
&\quad - \mathbb{E}_{q_m^n}[ \, \log \Pr(z_{T+1, m} = n \, | \,  \mathbf{I} )
]
\end{split}
\end{equation}
The desirable property of this loss function is as:
\begin{lemma}\label{lemma:bound}
The negative log-likelihood defined by Eq.~\eqref{eq:mix} is upper-bounded by the loss function Eq.~\eqref{eq:loss} in the EM process: 

\centering$-\log\prod\limits_{m} p(y_{T+1, m} \,|\mathbf{X}_{T,m} \,; \Theta) \leq \mathcal{L}(\Theta, \mathbf{I})$
\end{lemma}
The proof is provided in the supplementary material. 

 \begin{figure}[htbp]
     \vspace{-0pt}
     \centering
     \begin{subfigure}[t]{0.23\textwidth}
         \centering
         \includegraphics[width=0.95\textwidth]{figures/att_var-eps-converted-to.pdf}
         % \caption{}
     \end{subfigure}
     %~
     \begin{subfigure}[t]{0.24\textwidth}
         \centering
         \includegraphics[width=0.95\textwidth]{figures/att_var_temp-eps-converted-to.pdf}
         % \caption{}
     \end{subfigure}
     \caption{\small{Left: Histograms of variable attention at different epochs. Right: Histograms of temporal attention of variable ``P-temperature''. It is nontrivial to interpret variable and temporal importance from attention values on training instances.}
     }
     \vspace{-5pt}
     \label{fig:att_interpret}
 \end{figure}
Therefore, minimizing Eq.~\eqref{eq:loss} enables to simultaneously learn the network parameters and importance vectors without the need of post processing on trained networks.



% \tao{should clarify why we need to minimize this loss function, why it is fine to use EM, why EM framework works. We should clearly connect to the Section 3.2. The logic here is not clear.
% Also, why we can have such a design choice as Eq.11?
% }

In particular, in Eq.~\eqref{eq:loss} the first two terms
% , $\mathbb{E}_{q_m^n}[ \, \log p( y_{T+1, m} \, | \cdot) ]$ and $\mathbb{E}_{q_m^n}[ \, \Pr(z_{T+1, m} \, | \, \cdot)]$, 
are derived from the standard EM procedure.
For the last term $\mathbb{E}_{q_m^n}[ \, \log \Pr(z_{T+1, m} = n \, | \,  \mathbf{I} )$, intuitively it serves as a regularization on the posterior of latent variable $z_{T+1, m}$ and encourages individual instances to follow the global pattern $\mathbf{I}$, which parameterizes a discrete distribution on $z_{T+1, m}$. 
And $q^n_m$ represents the posterior of $z_{T+1, m}$ by Eq.~\eqref{eq:poster}:
\begin{equation}\label{eq:poster}
\textstyle
\begin{split}
\textstyle
& q^n_m  \coloneqq \Pr (z_{T+1, m}  = n | \, \mathbf{X}_{T, m}, y_{T+1, m} \, ; \Theta) \\
& \propto p(y_{T+1, m} | z_{T+1, m} = n, \mathbf{X}_{T, m} ) \cdot \Pr(z_{T+1, m} = n | \mathbf{X}_{T, m}) \\
& \approx p( y_{T+1, m} \, | \, z_{T+1, m} = n,  \mathbf{h}_T^n \oplus \mathbf{g}^n  ) \\
&\quad \cdot \Pr(z_{T+1, m} = n \, | \, \mathbf{h}_T^1 \oplus \mathbf{g}^1, \cdots, \mathbf{h}_T^N \oplus \mathbf{g}^N )
\end{split}
\end{equation}
During the training phase, network parameters $\Theta$ and importance vectors are alternatively learned. 
In a certain round of the loss function minimization, we first fix the current value of $\Theta$ and evaluate $q_m^n$ for the batch of data. 
Then, since the first two terms in the loss functions solely depend on network parameters $\Theta$, they are minimized via gradient descent to update $\Theta$. 
For the last term, fortunately we can derive a simple closed-form solution of $\mathbf{I}$ as:
\begin{equation}
\textstyle
\mathbf{I} = \frac{1}{M} \sum_m \mathbf{q}_m,  \text{    } \mathbf{q}_m = [q_m^1, \cdots, q_m^n]^{\top}
\end{equation}
, which takes into account both variable attention and predictive likelihood in the importance vector.

As for temporal importance, it can also be derived through EM, but it requires a hierarchical mixture. 
For the sake of computing efficiency, the variable-wise temporal importance vector is derived from attention values as follows:
\begin{equation}
\textstyle
\mathbf{T}^n =  \frac{1}{M} \sum_m \boldsymbol{\alpha}_m^n,  \text{    } \boldsymbol{\alpha}_m = [\alpha_{1, m}^n, \cdots, \alpha_{T, m}^n]^{\top}
\end{equation}
This process iterates until convergence.
After the training, we obtain the neural networks ready for predicting as well as the variable and temporal importance vectors.
Then, in the predicting phase, the prediction of $y_{T+1}$ is obtained by the weighted sum of means as:
\begin{small}
\begin{equation}
\textstyle
\hat{y}_{T+1} = \sum_n  \mu_n \cdot \Pr(z_{T+1} = n \, | \, \mathbf{h}_T^1 \oplus \mathbf{g}^1, \cdots, \mathbf{h}_T^N \oplus \mathbf{g}^N ) \,.
\end{equation}
\end{small}
\vspace{-0.8cm}

==> Exploring interpretable LSTM neural networks over multi-variable data/related.tex <==
\section{Related Work}
% In time series analysis, prediction with exogenous variables can formulated as an auto-regressive exogenous model or prediction modeles defined on exogenous variables.
% Vanilla RNNs have been used to study it in~\citep{zemouri2010defining, diaconescu2008use}, where interpretability was not investigated. 
% \citep{dipietro2017analyzing} studied the vanishing gradient problem of ARX RNN model via skip connections.
% To the best of our knowledge, this is the first work to explore the capability of recurrent neural networks for accurate forecasting, variable and temporal level importance interpreting simultaneously.

% --- backup reference list
% \citep{tank2017interpretable, tank2018neural}

% The interpretability of recurrent neural networks has attracted increasing interest. 
Recent research on the interpretable RNNs can be categorized into two groups: attention methods and post-analyzing on trained models.
Attention mechanism has gained tremendous popularity~\citep{xu2018raim, choi2018fine, guo2018interpretable, lai2017modeling, qin2017dual, cinar2017position, choi2016retain, vinyals2015pointer, bahdanau2014neural}.
However, current attention mechanism is mainly applied to hidden states across time steps.
\citet{qin2017dual, choi2016retain} built attention on conventional hidden states of encoder networks. 
Since the hidden states encode information from all input variables, the derived attention is biased when used to measure the importance of corresponding variables. 
The contribution coefficients defined on attention values is biased as well \citep{choi2016retain}. 
Moreover, weighting input data by attentions \citep{xu2018raim, qin2017dual, choi2016retain} does not consider the direction of correlation with the target, which could impair the prediction performance.
Current attention based methods seldom provide variable-wise temporal interpretability.

% and for multi-variable input sequence, it fails to characterize variable level importance. 
% Only some recent studies~\citep{qin2017dual, choi2016retain} attempted to develop attention on variables.

% , since it enables recurrent neural networks to select parts of hidden states as well as enhancing the interpretability


% Weighting input data overlooks the direction of correlation
% not unique, attention on individual training instances 

% \cite{qin2017dual} is \textcolor{red}{built upon encoder-decoder architecture, which used one network to learn weights for input variables first and then fed pre-weighted input data into another network to learn the relation between input and target variables}. 
% \cite{choi2016retain} pre-trained two recurrent neural networks to respectively derive weights on temporal steps and variables, which were then used to perform prediction.

% --- backup reference list:
% GeoMAN: Multi-level Attention Networks for Geo-sensory Time Series Prediction
% A Memory-Network Based Solution for Multivariate Time-Series Forecasting
% Hierarchical Attention-Based Recurrent Highway Networks for Time Series Prediction

% The success of attention mechanism in 
% encoder-decoder networks \cite{cho2014properties, cho2014learning, sutskever2014sequence}
% time series analysis \cite{choi2016retain, qin2017dual, cinar2017position}, \cite{qin2017dual}. 
% image processing~\cite{ba2014multiple,mnih2014recurrent,gregor2015draw,xu2015show}, 
% natural language processing~\cite{hermann2015teaching,rush2015neural,lin2017structured} and 
% speech recognition~\cite{chorowski2015attention}.
% sequence to sequence data \cite{cho2014properties, cho2014learning, sutskever2014sequence}, 
% Numerous research explored the interpretability of recurrent neural networks by 

% decomposition
% perturbation
% gradient
% relevance propagation

As for post-analyzing interpretation,~\citet{murdoch2018beyond, murdoch2017automatic, arras2017explaining} extracted temporal importance scores over words or phrases of individual sequences by decomposing the memory cells of trained RNNs.
In perturbation-based approaches perturbed samples might be different from the original data distribution~\citep{ribeiro2018anchors}.
Gradient-based methods analyze the features that output was most sensitive to~\citep{ancona2018towards, shrikumar2017learning}.
Above methods mostly focused on one type of importance and are computationally inefficient. They rarely enhance the predicting performance.

\citet{wavelet} focused on the importance of each middle layer to the output.
\citet{chu2018exact} proposed interpreting solutions for piece-wise linear neural networks.
% \citep{chu2018exact, foerster2017input} use piece-wise linear and affine transforamtion to a
% \citet{chu2018exact} proposed interpretating solutions for piece-wise linear neural networks.
\citet{foerster2017input} introduced input-switched linear affine transformations into RNNs to analyze the contribution of input steps, wihch could lead to the loss in prediction performance.
Our paper focuses on exploring the internal structure of LSTM so as to learn accurate forecasting and importance measures simultaneously.
% and the derived mixture attention and training method enable

% As for post-analyzing based interpretation,~\cite{murdoch2017automatic} extracted temporal importance scores over individual language sequences by decomposing the memory cells of trained LSTM.
% \cite{chu2018exact} proposed interpretation solutions for piece-wise linear neural networks.
% In~\cite{wavelet}, it quantified the importance of each middle layer to the output.
% \cite{foerster2017input} introduced input-switched affine transformations into RNN, which allowed to analyze the contribution of input steps via linear methods.
% Work on analyzing the contribution of words or phrases into prediction~\citep{murdoch2018beyond, arras2017explaining} essentially only captured the importance of steps as well.
% Our following proposed IMV-LSTM is a combination of attention and post-analyzing for multi-variable time series, where novel mixture attention enables fine-grained temporal and variable importance interpretation during the training. 
% In our IMV-LSTM, temporal and variable attention are jointly derived from variable-wise hidden states learned via one end-to-end network. The derived overall variable importance reflects the contribution into prediction by each variable.  

% decomposed LSTM outputs using telescoping sums of statistics
% computed from memory cells at different RNN steps.
% The decomposition is exact, but not in-unique and the authors
% justify it by demonstrating good performance of decision
% rules formed using the computed cell statistics.

% -- backup reference list:
% input switched rnn, multiplicative lstm for sequence modeling
% survey on variable importance

Another line of related research is about tensorization and decomposition of hidden states in RNNs. 
\citet{do2017matrix, novikov2015tensorizing} proposed to represent hidden states as matrices. 
\citet{he2017wider} developed tensorized LSTM to enhance the capacity of networks without additional parameters.
\citet{kuchaiev2017factorization, neil2016phased, koutnik2014clockwork} proposed to partition the hidden layer into separated modules with different updates. 
These hidden state tensors and update processes 
% (i.e. convolution operation or matrix multiplication) 
do not maintain variable-wise correspondence and lack the desirable interpretability.
% \tian{update}
% IMV-LSTM uses tensor-dot to derive cell update, in order to ensure each element in the tensorized hidden states encodes information from a certain variable for the subsequent mixture attention and interpretation. 

% In IMV-LSTM, hidden states are organized in a matrix, each element of which encodes information specific to an input variable. Meanwhile, the hidden states are correlatively updated such that inter-correlation among input variables is still captured.  

% Attention mechanism is originally proposed in the context of encoder-decoder networks 

% In time series analysis, this could be a concern since we usually expect to make predictions based upon a relatively long segment of the target series as well as driving series. 

% One problem with encoder-decoder networks is that their performance will deteriorate rapidly as the length of input sequence increases [Cho et al., 2014a]. 

% To resolve this issue, the attention-based encoder decoder network [Bahdanau et al., 2014] employs an attention mechanism to select parts of hidden states across all the time steps. 

% hierarchical attention network [Yang et al., 2016], which uses two layers of attention mechanism to select relevant encoder hidden states across all the time steps, was also developed. 

% Although attention-based encoderdecoder networks and hierarchical attention networks have shown their efficacy for machine translation, image captioning [Xu et al., 2015], and document classification, they may not be suitable for time series prediction. 

% This is because when multiple driving (exogenous) series are available, the network cannot explicitly select relevant driving series to make predictions. In addition, they have mainly been used for classification, rather than time series prediction.

% \citep{choi2016retain} develops two-level neural attention model for time series classification, trying to capture the influential time step and significant features.

% \citep{qin2017dual} proposes dual-stage attention-based recurrent neural network,
% where input attention mechanism on the encoder adaptively builds input features for each time step based on previous hidden state, while temporal attention mechanism selects relevant encoder hidden states across all time steps.



